GEOALIGN: Geometric Rollout Curation for Robust LLM Reinforcement Learning

Online reinforcement learning is widely used to align large language models (LLMs) with reward signals, yet training can be unstable under noisy or misspecified rewards. We identify a failure mode we call directional inconsistency: within a batch, a small set of high-reward rollouts induces representation-space preference directions that sharply disagree with the batch majority, resulting in high-variance and destabilizing updates. We propose geoalign, a lightweight plug-in for rollout curation in iterative policy optimization. Geoalign (i) forms within-prompt preference pairs, (ii) learns an online projector on per-rollout hidden states to concentrate reward-ordered displacement directions, and (iii) detects directionally inconsistent rollouts via their angular deviation from a batch consensus prototype and rectifies them with within-prompt stable alternatives. Geoalign is forward-pass only and adds negligible overhead. Across dialogue alignment with a learned reward model and mathematical reasoning with binary verified rewards, Geoalign improves final performance and reduces training oscillation, outperforming PF-PPO, PAR, PODS, and Seed-GRPO. These results suggest latent directional consensus as an effective reliability signal for online LLM RL.

==> ICML/sec/bak/0123_method.tex <==
% \iffalse 一些要点：

% 围绕“几何一致性 vs 冲突更新”的视觉与逻辑主线展开

% e.g., 

% 3.1 Problem Formulation: Directional Inconsistency in Online RL
% Intuition: Just as in contrastive learning, we care not just about individual samples, but about the relative geometry between them.

% 3.2 Geometric Prototype: Capturing Consensus Improvement Direction
% Why EMA? 避免 prototype 被单个 outlier 扭曲；体现“evolving consensus”

% 3.3 Conflict-Aware Rollout Weighting
% Key Insight: We don’t discard samples—we softly suppress those that “pull the policy backward”

% 3.4 Integration with Policy Gradient Objectives
% Emphasize: No extra backward pass, no reference model, no gradient computation → fully online

% 3.5 (Potential, theoretical analysis)


% 技术性checklist
% - 明确定义 improvement direction，譬如 Δz = z⁺ - z⁻ 
% - prototype 是 EMA of recent Δz，不是静态中心
% - conflict = negative cosine similarity，soft downweighting
% - 强调 no extra compute（representations reused）
% - Figure 1 直观展示 conflict vs alignment
% - 伪代码体现 online, plug-and-play 特性
% \fi

\section{GeoAlign: Online Calibration via Latent
Directional Consistency}

We first discuss the design motivation behind GeoAlign, then describe its algorithmic components in Fig. \ref{fig:overall}.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{ICML/Fig/Process_Figure.pdf}
  \caption{\textbf{GeoAlign overview.} At each iteration, we form within-prompt preference displacements from low-reward to high-reward rollouts, project them onto a reward-sensitive manifold, construct a batch-wise consensus prototype, score rollouts by directional inconsistency, and rectify the experience buffer by replacing anomalous experiences with stable ones from the same prompt (equivalently setting their optimization weight to zero) before running the RL update (e.g., PPO/GRPO).}
  \label{fig:overall}
\end{figure*}

% To address training instability caused by noisy reward signals in online reinforcement learning (e.g., reward hacking), we propose GeoAlign. Instead of relying solely on scalar rewards, GeoAlign analyzes the latent improvement geometry of policy updates in the representation space to identify and filter out anomalous update directions. Analogous to contrastive learning, the method focuses not just on individual samples but on their relative geometric relationships.

% GeoAlign operates as a plug-and-play module comprising four stages:
% (1) Preference manifold sampling,
% (2) Dynamic semantic projection,
% (3) Geometric prototype construction and anomaly detection,
% (4) Geometry-aware policy update.

\subsection{Preliminary}


\subsection{Why Directional Consistency Helps: A Semi-Theoretical View}
\label{sec:theory_insight}
%  进一步分析方向（用来写实验/附录分析，增强可信度）下面这些是“写得更学术”的可操作分析路线（很多不需要重训）：

% 1) **低维子空间而非单一方向**  
%    - 现在用 centroid direction。更强的说法是：投影后向量在单位球面上集中在一个小 cap，或集中在 top-r PCA 子空间。  
%    - 分析：对 projected vectors 做 PCA，报告解释方差比（EVR），看 r=1/2/4 时覆盖多少；随训练演化是否更集中。  
%    - 若发现 r>1 明显更好，未来可扩展为“prototype subspace”，异常度用到子空间距离。

% 2) **update rotation 的直接量化（强说服力）**  
%    - 不重训：在每步，记录“全样本 GRPO 梯度方向” vs “去掉 top-α outliers 后的梯度方向”的夹角（或 cosine）。  
%    - 结论若是：少量 outliers 会显著 rotate update，等价证明了“高杠杆点”。

% 3) **鲁棒统计的形式化对照（method 更站得住）**  
%    - 把当前硬阈值看成 Tukey / trimmed estimator 的特例。  
%    - 做对照：hard drop vs soft weight \(w=\exp(-\lambda \alpha)\)，看稳定性/最终性能/多样性 tradeoff。

% 4) **“reward 高但方向不一致”的案例归因**  
%    - 抽 top anomaly 但 reward 排名前列的样本，做 LLM judge 或人工标注，展示其是“投机/格式/偏离任务”等。  
%    - 这能回答“为什么 scalar reward 不够”。

% 5) **一致性假设的边界条件**  
%    - 找一些 batch 内本来就多模态（例如既需要 helpful 又需要 harmless 相互拉扯），看 prototype 是否变成 subspace。  
%    - 给出失败模式：当任务目标本身多峰时，单 prototype 会过度过滤；你们可以用 mixture prototypes 作为 future work。


GeoAlign is motivated by a simple geometric perspective on on-policy RL fine-tuning.
Consider one RL iteration with a batch of prompts $\{x_i\}_{i=1}^N$, and $K$ rollouts per prompt sampled from the current policy $\pi_\theta$.
Let $h_\theta(x,y)\in\mathbb{R}^d$ denote a pooled hidden representation of the rollout (e.g., last-layer mean pooling), and define a \emph{preference displacement} for a within-prompt preference pair $(y_w,y_l)$ as
$\delta = h_\theta(x,y_w) - h_\theta(x,y_l)$.

\paragraph{Insight 1 (local improvement directions concentrate).}
If the reward model is approximately consistent within the current batch (i.e., it induces a stable notion of ``better'' for most prompts), then improving reward often corresponds to modifying a limited set of high-level attributes (helpfulness, harmlessness, correctness, etc.).
Under mild smoothness of representations, this implies that, within a single iteration, many preference displacements $\{\delta_j\}_{j\in\mathcal{P}}$ tend to share a dominant direction or a low-dimensional subspace, up to task-irrelevant variation.
Empirically, our online projector $\mathcal{M}_\psi$ makes this concentration explicit by suppressing nuisance factors and producing projected directions that exhibit high cosine agreement (Sec.~\ref{exp:ProjectorNecessary}).

\paragraph{Insight 2 (directional outliers inflate update variance).}
Policy gradient methods update parameters using a weighted average of per-sample learning signals.
When a small fraction of rollouts induces preference displacements that are nearly orthogonal (or adversarial) to the batch-wise dominant direction, their corresponding gradient contributions behave like \emph{high-leverage} points: they can substantially rotate the aggregated update direction and increase update variance, causing oscillatory training dynamics even if their scalar rewards are high.
Importantly, PPO/GRPO clipping constrains the \emph{magnitude} of each sample's contribution through probability ratios, but does not prevent a small set of samples from rotating the aggregated update direction.

\paragraph{Insight 3 (GeoAlign as robust estimation).}
Viewed abstractly, one iteration of policy optimization can be seen as estimating a latent ``consensus improvement'' direction from noisy directional observations.
GeoAlign computes a consensus prototype $v_{\mathrm{proto}}$ and suppresses rollouts with large angular deviation from it, analogous to robust $M$-estimation where outliers receive bounded influence.
This perspective explains why GeoAlign improves stability under reward corruption: directionally inconsistent samples are treated as outliers in the space of improvement directions, rather than being trusted solely based on scalar reward values.


\subsection{Manifold Sampling of Preference Pairs in Latent Space}
\label{sec:pair_sampling}

We consider an online RL setup where, at each iteration, a policy $\pi_\theta$ generates $K$ rollouts $\{y_{i,1}, \dots, y_{i,K}\}$ for a prompt $x_i \sim \mathcal{D}$, each receiving a scalar reward $r_{i,k}$.
We extract the pooled hidden representation $\mathbf{h}_{i,k} \in \mathbb{R}^d$ for each rollout (e.g., from the last transformer layer).

Rather than analyzing individual points, we focus on the \textit{directions of improvement}.
For each prompt, we construct a set of local preference pairs based on strict reward ranking:
\begin{equation}
\mathcal{P} = \bigcup_{i} \left\{ (i,k,\ell) \mid r_{i,k} > r_{i,\ell} \right\}.
\end{equation}
For any $(i,k,\ell) \in \mathcal{P}$, the raw difference vector
\begin{equation}
\boldsymbol{\delta}^{\text{raw}}_{i,k,\ell} = \mathbf{h}_{i,k} - \mathbf{h}_{i,\ell}
\end{equation}
represents a transition from a lower-reward behavior to a higher-reward one. However, in high-dimensional language models, these raw directions are often noisy and entangled with task-irrelevant linguistic variance, motivating a projection step.
% \subsection{Manifold Sampling of Preference Pairs in Latent Space}

% We consider an online RL setup where, at each iteration, a policy $\pi_\theta$ generates $K$ rollouts $\{y_{i,1}, \dots, y_{i,K}\}$ for a prompt $x_i \sim \mathcal{D}$, each receiving a scalar reward $r_{i,k}$.
% To capture the latent dynamics of the policy, we extract the pooled hidden representation $\mathbf{h}_{i,k} \in \mathbb{R}^d$ for each rollout (e.g., from the last transformer layer).

% Rather than analyzing individual points, we focus on the \textit{directions of improvement}. For each prompt, we construct a set of local preference pairs based on reward ranking:
% \begin{equation}
% \mathcal{P} = \bigcup_{i} \left\{ (y_w, y_l) \mid r(y_w) > r(y_l), \; y_w, y_l \sim \pi_\theta(\cdot|x_i) \right\}.
% \end{equation}
% For any pair $(y_w, y_l) \in \mathcal{P}$, the raw difference vector $\boldsymbol{\delta}_{\text{raw}} = \mathbf{h}(y_w) - \mathbf{h}(y_l)$ represents a transition from a lower-reward behavior to a higher-reward one. However, in high-dimensional language models, this raw direction is often noisy, necessitating a dedicated projection mechanism.


\subsection{Directional Distillation for Improvement Manifolds}
\label{sec:projector}
The raw hidden representations of the policy are inherently entangled with task-irrelevant linguistic variances (e.g., lexical noise or stylistic bias), which mask the underlying geometry of policy improvement. To isolate the effective update direction, we introduce a lightweight projector $\mathcal{M}_\psi: \mathbb{R}^d \rightarrow \mathbb{R}^{d'}$, which maps raw latent differences onto a lower-dimensional, reward-sensitive manifold.

\paragraph{Online projector training.}
We update $\mathcal{M}_\psi$ online using within-batch preference pairs only.
For each $(i,k,\ell)\in\mathcal{P}$, define a normalized positive direction
$u^+=\mathrm{norm}(\mathbf{h}_{i,k}-\mathbf{h}_{i,\ell})$ and a normalized negative direction
$u^-=\mathrm{norm}(\mathbf{h}_{i,\ell}-\mathbf{h}_{i,k})$.
We train $\mathcal{M}_\psi$ with a lightweight linear probe $w\in\mathbb{R}^{d'}$ using BCE:
\begin{equation}
\label{eq:projector}
\begin{split}
\mathcal{L}_{\mathrm{map}}(\psi,w)
=&-\mathbb{E}_{(i,k,\ell)\in\mathcal{P}}
\Big[\log\sigma\big(w^\top \mathcal{M}_\psi(u^+)\big)
\\
&\quad\quad\quad+
\log\big(1-\sigma\big(w^\top \mathcal{M}_\psi(u^-)\big)\big)\Big].
\end{split}
\end{equation}

\noindent\textbf{Implementation details.}
$\mathcal{M}_\psi$ is a two-layer MLP with ReLU and dropout (0.1), trained for 50 steps per RL iteration with a cosine learning-rate schedule (initial LR $10^{-3}$).
We use a 9:1 train/validation split of $\mathcal{P}$ within each iteration to monitor projector generalization (reported in Sec.~\ref{exp:ProjectorNecessary}).
After updating, the probe $w$ is discarded.

\paragraph{Projected improvement directions.}
We compute normalized projected directions for each preference pair:
\begin{equation}
\mathbf{v}_{i,k,\ell} = \mathrm{norm}\!\left(\mathcal{M}_\psi\big(\mathrm{norm}(\boldsymbol{\delta}^{\text{raw}}_{i,k,\ell})\big)\right).
\end{equation}
Empirically, this projection is critical for revealing directional concentration and making a simple prototype robust (Fig.~\ref{fig:ProjectorNecessary}).

\hl{
% another version of Eq.3 and Eq.4 for mathmatical beauty (namely geometric filter), to check and discuss by ting & zhenqin
\paragraph{Directional Subspace Learning.}
To distill the reward-sensitive manifold from high-dimensional noise, $\mathcal{M}_\psi$ is trained to maximize the separability of preference directions. Let $\boldsymbol{u}_{i,k,\ell} = \frac{\boldsymbol{h}_{i,k} - \boldsymbol{h}_{i,\ell}}{\|\boldsymbol{h}_{i,k} - \boldsymbol{h}_{i,\ell}\|_2}$ be the unit displacement vector. We minimize:
\begin{equation}
\mathcal{L}_{\text{distill}}(\psi, \boldsymbol{w}) = -\sum_{(i,k,\ell) \in \mathcal{P}} \left[ \log \sigma(\boldsymbol{w}^\top \mathcal{M}_\psi(\boldsymbol{u}_{i,k,\ell})) + \log (1 - \sigma(\boldsymbol{w}^\top \mathcal{M}_\psi(-\boldsymbol{u}_{i,k,\ell}))) \right]
\end{equation}
where $\mathcal{M}_\psi$ acts as a \textit{geometric filter} that suppresses directions orthogonal to the local improvement manifold.

\paragraph{Geometric Inconsistency Metric.}
We define the Geometric Deviation Index (GDI) for a rollout $y_{i,k}$ as the mean angular distance from the batch consensus prototype $\boldsymbol{v}_{\text{proto}}$:
\begin{equation}
\text{GDI}(i,k) = \frac{1}{|\mathcal{P}_{i,k}|} \sum_{(k,\ell) \in \mathcal{P}_{i,k}} \left( 1 - \frac{\langle \mathcal{M}_\psi(\boldsymbol{u}_{i,k,\ell}), \boldsymbol{v}_{\text{proto}} \rangle}{\|\mathcal{M}_\psi(\boldsymbol{u}_{i,k,\ell})\| \|\boldsymbol{v}_{\text{proto}}\|} \right)
\end{equation}
Samples with extreme GDI values are identified as \textit{directional outliers}, likely representing reward-hacking trajectories that deviate from the systemic improvement of the policy.


\subsection{Geometric Prototype and Anomaly Detection}
\label{sec:anomaly}

With the projected manifold, we quantify directional consistency.
We define the consensus improvement direction (geometric prototype) as the normalized centroid of projected directions:
\begin{equation}
\mathbf{v}_{\text{proto}} = \mathrm{norm} \left( \frac{1}{|\mathcal{P}|} \sum_{(i,k,\ell)\in\mathcal{P}} \mathbf{v}_{i,k,\ell} \right).
\end{equation}
The unit-normalization ensures that the prototype is determined by the majority consensus of directions rather than magnitudes.

\paragraph{Pair-level deviation score.}
For each preference pair, we compute a cosine-based anomaly score:
\begin{equation}
s_{i,k,\ell} = 1 - \cos(\mathbf{v}_{i,k,\ell}, \mathbf{v}_{\text{proto}}).
\end{equation}
When $s_{i,k,\ell}\approx 0$, the improvement direction aligns with consensus; large values indicate orthogonal/adversarial deviation.

\paragraph{Rollout-level inconsistency score.}
Since optimization is performed at the rollout level, we aggregate pairwise scores back to responses.
For any response $y_{i,k}$, define
\begin{equation}
\alpha_{i,k} = \frac{1}{N_{i,k}}
\sum_{\ell: (i,k,\ell)\in\mathcal{P}} s_{i,k,\ell}
+
\frac{1}{N_{i,k}}
\sum_{\ell: (i,\ell,k)\in\mathcal{P}} s_{i,\ell,k},
\end{equation}
where $N_{i,k}$ is the total number of preference pairs in which $y_{i,k}$ participates.
This aggregation evaluates a rollout through multiple preference-induced interactions rather than as an isolated sample.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{ICML/Fig/anomaly_rank_plot_rm.png}
        \caption{Under a continuous reward model proxy.}
        \label{fig:latent_continuous}
    \end{subfigure}
    \vspace{0.5em}
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{ICML/Fig/anomaly_rank_plot_math.png}
        \caption{With discrete binary rewards.}
        \label{fig:latent_discrete}
    \end{subfigure}
    \caption{\textbf{Anomaly score--rank distribution.} Geometric inconsistency exhibits a long-tail pattern, motivating targeted intervention on a small subset of rollouts.}
    \label{fig:anomaly_score_rank}
\end{figure}

\subsection{Geometry-Aware Experience Rectification}
\label{sec:rectify}

GeoAlign mitigates the effect of geometric outliers while maintaining gradient density by rectifying experiences in the buffer.
We use a dual-threshold filter based on (i) a \emph{budget} $k$ and (ii) a percentile threshold $\tau_\alpha$ over anomaly scores.
Specifically, we mark at most a fraction $k$ of rollouts in a batch as anomalous (we use $k=0.1$ of total rollouts), and require $\alpha_{i,k}$ to exceed the $\tau_\alpha$-th percentile (we tune $\tau_\alpha\in[0.2,0.6]$ depending on task/model; see Appendix~\ref{appendix:train_details}).

For each prompt $x_i$, let $\mathcal{Y}_{\text{anom}}(i)$ denote the anomalous rollouts and $\mathcal{Y}_{\text{stable}}(i)$ the remaining stable ones.

\paragraph{Replacement within the same prompt.}
For each anomalous rollout in $\mathcal{Y}_{\text{anom}}(i)$, we replace it in the experience buffer by sampling a representative $y^*$ from $\mathcal{Y}_{\text{stable}}(i)$ following a Best-Random strategy~\cite{zhang2024policy}:
\begin{equation}
\small
P(y^* = y_j \mid y_j \in \mathcal{Y}_{\text{stable}}(i)) = 
\begin{cases}
0.5, & \text{if } y_j = \displaystyle \arg\max_{y \in \mathcal{Y}_{\text{stable}}(i)} r(y), \\[6pt]
\dfrac{0.5}{|\mathcal{Y}_{\text{stable}}(i)| - 1}, & \text{otherwise}.
\end{cases}
\end{equation}
Operationally, this replacement is equivalent to assigning zero optimization weight to the anomalous experience while keeping the effective batch size unchanged, which stabilizes policy updates without discarding the whole prompt's data.

\input{ICML/sec/algorithom}

\subsection{Practical Considerations}
\label{sec:practical}
\paragraph{Ties and empty preference sets.}
If a prompt yields no strictly ordered preference pairs (e.g., all binary rewards are tied), then $\mathcal{P}_i=\emptyset$ and GeoAlign skips scoring for that prompt, leaving its rollouts unchanged.
If the entire batch yields $|\mathcal{P}|=0$, GeoAlign becomes an identity mapping for that iteration.

\paragraph{Complexity.}
Forming within-prompt preference pairs costs $O(NK^2)$ and scoring costs $O(|\mathcal{P}|d')$ per iteration.
With $K\le 16$ and a small projector, the overhead is negligible relative to rollout generation and the main RL update (profiling in Appendix~\ref{appendix:profiling}). % TODO: add appendix label






% \paragraph{Online Projector Training.}
% We update $M_\psi$ online using within-batch preference pairs only.
% For each $(i,k,\ell)\in\mathcal{P}$, define a positive direction
% $u^+=h_{i,k}-h_{i,\ell}$ and a negative direction $u^-=h_{i,\ell}-h_{i,k}$.
% We train $M_\psi$ with a lightweight linear probe $w\in\mathbb{R}^{d'}$ using BCE:
% \begin{equation}
% \label{eq:projector}
% \begin{split}
% \mathcal{L}_{\mathrm{map}}(\psi,w)
% =&-\mathbb{E}_{(i,k,\ell)\in\mathcal{P}}
% \Big[\log\sigma\big(w^\top M_\psi(u^+)\big)
% \\
% &\qquad\qquad\qquad\quad+
% \log\big(1-\sigma\big(w^\top M_\psi(u^-)\big)\big)\Big].
% \end{split}
% \end{equation}

% Through this objective, the auxiliary probe $\mathbf{w}$ guides $\mathcal{M}_\psi$ to align its output space with the axis of reward improvement. 
% After the update, the probe $\mathbf{w}$ is discarded, and we use the normalized projected vector $\mathbf{v}_{j} = \text{norm}(\mathcal{M}_\psi(\boldsymbol{\delta}_{\text{raw}, j}))$ as the refined representation for the $j$-th preference pair.



% \hl{This projection is critical for rectifying the latent space, ensuring that consensus analysis is conducted on a purified improvement manifold (see Sec.}~\ref{exp:ProjectorNecessary}\hl{).
% Moreover, despite the online training, the computational overhead is negligible compared to the primary RL process (see Appendix~\ref{} for detailed profiling).
% }


% % \subsection{Geometric Prototype and Anomaly Measurement}
% \subsection{Geometric Prototype and Anomaly Detection}
% \label{sec:anomaly}
% With the projected manifold, we quantify directional consistency. We hypothesize that legitimate policy improvements should share a common latent direction (consensus).

% \paragraph{Consensus Prototype.}
% We define the consensus improvement direction, $\mathbf{v}_{\text{proto}}$, as the centroid of all valid preference pairs in the batch:
% \begin{equation}
% \mathbf{v}_{\text{proto}} = \text{norm} \left( \frac{1}{|\mathcal{P}|} \sum_{j \in \mathcal{P}} \mathbf{v}_j \right).
% \end{equation}
% The $\text{norm}(\cdot)$ operation unit-normalizes each vector to ensure equal contribution, allowing $\mathbf{v}_{\text{proto}}$ to be determined by the majority consensus of directions rather than individual magnitudes, thereby avoiding distortion by extreme noise. The prototype summarizes the dominant direction along which the current policy improves reward under the present data distribution. It is updated dynamically at each step using the current batch, serving as a first-order local approximation of the dominant improvement direction under the current policy and data distribution.



% \paragraph{Rollout-Level Inconsistency Score.}
% We first quantify the directional deviation of each preference pair j $\in \mathcal{P}$ relative to the consensus prototype via a cosine-based anomaly score:
% \begin{equation}
% s_j = 1 - \cos(\mathbf{v}_j, \mathbf{v}_{\text{proto}}),
% \end{equation}
% where $\mathbf{v}_j$ denotes the projected vector of pair j. When $s_j \approx 0$, the improvement direction is well aligned with the group consensus and thus provides a high-confidence learning signal. In contrast, large values of $s_j$ signify a geometric divergence, where a trajectory moves orthogonally or adversarially to the collective improvement manifold. Such directional conflicts may flag instances of reward hacking, where the model exploits non-generalizable latent shortcuts.

% Since optimization is performed at the rollout level, we aggregate pairwise anomaly scores back to individual responses. For any response y, its geometric inconsistency score $\alpha(y)$ is defined as the average anomaly score across all preference pairs in which it participates:

% \begin{equation}
% \bar{\alpha}(y) = \frac{1}{N_y} \sum_{j \in \mathcal{P}, y \in j} s_j,
% \end{equation}

% where $N_y = |\{j \in \mathcal{P} : y \in j\}|$ denotes the total number of preference pairs containing response $y$. 
% Through this aggregation, GeoAlign no longer treats a rollout as an isolated sample, but evaluates it through its interactions with multiple preference-induced directions.

% The resulting score $\alpha(y)$ serves as a conflict index: a high $\alpha(y)$ indicates that on average, the response exhibits a strong tendency to induce improvement directions that deviate from the batch-level consensus.
% This mechanism essentially quantifies the degree of localized geometric distortion caused by a specific response; by accumulating deviations across multiple pairings, we amplify the signal of singular directions that would otherwise be masked by scalar reward values.

% \input{ICML/sec/algorithom}


% \subsection{Geometry-Aware Policy Update}
% The ultimate utility of GeoAlign lies in its ability to translate geometric measurements into a robust policy update. Empirical observation of the anomaly scores $\alpha(y)$ across a training batch reveals a characteristic long-tail distribution. This indicates that directional conflict is not a uniform noise distribution; rather, it is concentrated within a small subset of singular samples that may promote updates adversarial to the consensus improvement manifold.

% \begin{figure}[htbp]
%     \centering

%     \begin{subfigure}{\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{ICML/Fig/anomaly_rank_plot_rm.png}
%         \caption{Under a Continuous Reward Model Proxy}
%         \label{fig:latent_continuous}
%     \end{subfigure}

%     \vspace{0.5em} % 调整上下子图间距，可按需改

%     \begin{subfigure}{\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{ICML/Fig/anomaly_rank_plot_math.png}
%         \caption{With Discrete Binary Rewards}
%         \label{fig:latent_discrete}
%     \end{subfigure}

%     \caption{Anomaly Score--Rank Distribution}
%     \label{fig:anomaly_score_rank}
% \end{figure}

% \hl{Empirically, we validate this interpretation through targeted ablation studies, including reversed weighting of high-$\alpha(y)$ samples and explicitly constructed directionally inconsistent pairs in Section} \ref{} and \ref{}.


% To mitigate the destabilizing impact of these geometric outliers while maintaining gradient density, we apply a geometry-guided resampling mechanism. Rather than simply discarding anomalous signals—which reduces sample efficiency—we reassign the optimization weight of flagged trajectories to more stable counterparts within the same prompt's rollout set. Specifically, we define a geometric weighting function $w(y)$ using a dual-threshold filter (percentile $\tau_\alpha$ and budget $k$):
% \begin{equation}
%     w(y) = \begin{cases} 0 & \text{if } \alpha(y) > \text{Threshold}(\tau_\alpha, k) \\ 1 & \text{otherwise} \end{cases}, 
% \end{equation}

% where the threshold is chosen to target only the head of the long-tail distribution, thereby limiting intervention to extreme geometric outliers and avoiding excessive suppression of potentially beneficial diversity.



% For trajectories where $w(y)=0$ (the set $\mathcal{Y}_{\text{anom}}$), we reallocate their gradient contribution to a consensus representative $y^*$ drawn from the stable set $\mathcal{Y}_{\text{stable}} = \{y \mid w(y)=1\}$. Inspired by the Best-Random strategy~\cite{zhang2024policy}, $y^*$ is sampled according to:
% \begin{equation}
% P(y^* = y_i \mid y \in \mathcal{Y}_{\text{anom}}) =
% \begin{cases}
% 0.5, & \text{if } y_i = \displaystyle \arg\max_{y \in \mathcal{Y}_{\text{stable}}} r(y), \\[6pt]
% \dfrac{0.5}{|\mathcal{Y}_{\text{stable}}| - 1}, & \text{otherwise}.
% \end{cases}
% \end{equation}

% Here, $\mathcal{Y}_{\text{stable}}$ denotes the set of rollouts that align with the geometric prototype, i.e., $w(y)=1$. By selectively intervening on a small number of rollouts with extreme directional conflict, GeoAlign reduces the influence of destabilizing updates and improves training robustness under noisy reward supervision.


% \daoyuan{
% % LLM-helped-version
% % =========================
% % GeoAlign Method (Replace)
% % =========================
% \section{GeoAlign: Online Calibration via Latent Directional Consistency}
% \label{sec:geoalign}

% \subsection{Setup and Notation}
% \label{sec:geoalign-setup}

% We consider online reinforcement learning for language models, where a policy
% $\pi_\theta(y\mid x)$ is optimized using a scalar reward function $R(x,y)$ (e.g., a reward model).
% At each iteration, we sample $N$ prompts $\{x_i\}_{i=1}^N \sim \mathcal{D}$ and generate $K$ rollouts per prompt:
% $y_{i,k} \sim \pi_\theta(\cdot\mid x_i)$ for $k\in[K]$.
% Each rollout receives a reward $r_{i,k}=R(x_i,y_{i,k})$.

% \paragraph{Representations.}
% For each prompt--response pair $(x_i,y_{i,k})$, we extract a pooled hidden representation
% $h_{i,k}\in\mathbb{R}^{d}$ from the current policy model.
% We denote this extraction as
% \begin{equation}
% h_{i,k} \;=\; \textsc{PoolHidden}(\pi_\theta, x_i, y_{i,k}),
% \end{equation}
% where \textsc{PoolHidden} is a deterministic pooling function over token-level hidden states
% (\TODO{specify: last token / mean pooling / attention pooling; which layer; length normalization}).
% We form the on-policy batch
% \begin{equation}
% \mathcal{B}=\{(x_i,y_{i,k},r_{i,k},h_{i,k})\}_{i=1..N,k=1..K}.
% \end{equation}

% \subsection{Definitions: Latent Improvement Directions and Directional Consistency}
% \label{sec:geoalign-definitions}

% GeoAlign is motivated by the observation that, within a minibatch, some high-reward rollouts may induce
% \emph{directionally inconsistent} improvement signals in representation space (e.g., due to reward model errors
% or spurious shortcuts). We quantify this inconsistency geometrically and use it to calibrate online experience.

% \paragraph{Preference pairs.}
% For each prompt $x_i$, we form an ordered set of preference pairs based on reward ranking:
% \begin{equation}
% \mathcal{P}_i=\{(k,\ell): r_{i,k} > r_{i,\ell}\},\qquad
% \mathcal{P}=\bigcup_{i=1}^N \{(i,k,\ell): (k,\ell)\in\mathcal{P}_i\}.
% \end{equation}

% \paragraph{Raw improvement direction.}
% For each preference pair $(i,k,\ell)\in\mathcal{P}$ (where $k$ wins over $\ell$), define the raw improvement vector
% \begin{equation}
% \delta^{\mathrm{raw}}_{i,k\ell}= h_{i,k}-h_{i,\ell}\in\mathbb{R}^{d}.
% \end{equation}

% \paragraph{Direction projector (optional but used in our default).}
% To reduce task-irrelevant variation in raw directions, we employ a lightweight projector
% $M_\psi:\mathbb{R}^d\to\mathbb{R}^{d'}$ and map raw directions to a reward-sensitive subspace:
% \begin{equation}
% \delta_{i,k\ell}=M_\psi(\delta^{\mathrm{raw}}_{i,k\ell})\in\mathbb{R}^{d'}.
% \end{equation}
% We use unit normalization for angular comparisons:
% \begin{equation}
% \tilde\delta_{i,k\ell}=\frac{\delta_{i,k\ell}}{\|\delta_{i,k\ell}\|+\epsilon},
% \end{equation}
% with a small $\epsilon>0$ for numerical stability.

% \paragraph{Consensus improvement prototype.}
% Given all preference-induced directions in the batch, we define the (unit) consensus prototype as
% \begin{equation}
% \label{eq:proto}
% v_{\mathrm{proto}} \;=\;
% \frac{\sum_{(i,k,\ell)\in\mathcal{P}} \tilde\delta_{i,k\ell}}
% {\left\|\sum_{(i,k,\ell)\in\mathcal{P}} \tilde\delta_{i,k\ell}\right\|+\epsilon}
% \;\in\;\mathbb{R}^{d'}.
% \end{equation}
% Intuitively, $v_{\mathrm{proto}}$ summarizes the dominant latent direction shared by most preference comparisons
% in the current on-policy batch.

% \paragraph{Pair-level anomaly score.}
% We quantify how much each preference pair deviates from the consensus via cosine anomaly:
% \begin{equation}
% \label{eq:pair-anom}
% s_{i,k\ell} \;=\; 1-\langle \tilde\delta_{i,k\ell}, v_{\mathrm{proto}}\rangle\in[0,2].
% \end{equation}
% Smaller $s_{i,k\ell}$ indicates higher directional consistency.

% \paragraph{Rollout-level inconsistency score.}
% Since policy optimization operates on rollouts, we aggregate pair-level anomalies to each rollout $(i,k)$.
% Let $\mathcal{P}(i,k)$ denote all preference pairs in which rollout $(i,k)$ participates (either as winner or loser):
% \begin{equation}
% \mathcal{P}(i,k)=\{(i,k,\ell)\in\mathcal{P}\}\cup\{(i,\ell,k)\in\mathcal{P}\}.
% \end{equation}
% We define the rollout inconsistency score as the \emph{mean} anomaly to avoid degree bias:
% \begin{equation}
% \label{eq:alpha}
% \alpha_{i,k} \;=\; \frac{1}{|\mathcal{P}(i,k)|}\sum_{p\in\mathcal{P}(i,k)} s_p.
% \end{equation}
% (\TODO{If you insist on sum aggregation, replace mean by sum and justify degree bias in experiments.})

% \subsection{Algorithm: GeoAlign Rectification Module}
% \label{sec:geoalign-algorithm}

% GeoAlign is a plug-and-play module that takes an on-policy batch $\mathcal{B}$ and outputs a rectified batch
% $\mathcal{B}_{\mathrm{rect}}$ by intervening on a small fraction of directionally inconsistent rollouts.
% It consists of four steps: (i) preference-pair construction, (ii) projector update, (iii) prototype and anomaly
% estimation, and (iv) geometry-aware resampling.

% \paragraph{Training the projector $M_\psi$.}
% We update $M_\psi$ online using within-batch preference pairs only.
% For each $(i,k,\ell)\in\mathcal{P}$, define a positive direction
% $u^+=h_{i,k}-h_{i,\ell}$ and a negative direction $u^-=h_{i,\ell}-h_{i,k}$.
% We train $M_\psi$ with a lightweight linear probe $w\in\mathbb{R}^{d'}$ using BCE:
% \begin{equation}
% \label{eq:projector}
% \begin{split}
% \mathcal{L}_{\mathrm{map}}(\psi,w)
% =&-\mathbb{E}_{(i,k,\ell)\in\mathcal{P}}
% \Big[\log\sigma\big(w^\top M_\psi(u^+)\big)
% \\
% &\qquad\qquad\qquad\quad+
% \log\big(1-\sigma\big(w^\top M_\psi(u^-)\big)\big)\Big].
% \end{split}
% \end{equation}
% After the update, we discard $w$ and use $M_\psi(\cdot)$ as the direction mapping.
% (\TODO{Specify: update steps $S$, LR, whether warmup/freeze, projector architecture and $d'$.})

% \paragraph{Dual-threshold anomaly filtering.}
% Empirically, $\{\alpha_{i,k}\}$ exhibits a long-tail distribution; thus we only intervene on the most inconsistent
% rollouts.
% Let $\mathrm{Percentile}(\{\alpha\},\tau_\alpha)$ be a percentile threshold, and let $k_{\max}$ be a budget on the
% maximum number of modified rollouts per batch.
% We flag rollouts by
% \begin{equation}
% \label{eq:dual-threshold}
% \mathcal{Y}_{\mathrm{anom}}
% =
% \left\{(i,k)\;\middle|\;
% \alpha_{i,k}\ge \mathrm{Percentile}(\{\alpha\},\tau_\alpha),\;
% (i,k)\in \mathrm{TopK}(\{\alpha\},k_{\max})
% \right\}.
% \end{equation}
% All non-flagged rollouts are considered stable: $\mathcal{Y}_{\mathrm{stable}}=\{(i,k)\}\setminus\mathcal{Y}_{\mathrm{anom}}$.

% \paragraph{Prompt-wise resampling within stable set.}
% For each flagged rollout $(i,k)\in\mathcal{Y}_{\mathrm{anom}}$, we resample a replacement rollout from the same prompt
% to preserve prompt-conditional distribution.
% Let $\mathcal{S}_i=\{k':(i,k')\in\mathcal{Y}_{\mathrm{stable}}\}$ denote stable indices for prompt $x_i$.
% We sample $k^\star\in\mathcal{S}_i$ via a Best-Random (BR) distribution biased towards the highest reward stable rollout:
% \begin{equation}
% \label{eq:br}
% \mathbb{P}(k^\star=k'\mid i)=
% \begin{cases}
% 0.5,& k'=\arg\max_{j\in\mathcal{S}_i} r_{i,j},\\[4pt]
% \frac{0.5}{|\mathcal{S}_i|-1},& \text{otherwise}.
% \end{cases}
% \end{equation}
% Then we replace $(y_{i,k},h_{i,k},r_{i,k})\leftarrow (y_{i,k^\star},h_{i,k^\star},r_{i,k^\star})$.
% The rectified batch $\mathcal{B}_{\mathrm{rect}}$ is then fed to any policy-gradient update (PPO/GRPO/etc.).

% \paragraph{Pseudocode.}
% Algorithm~\ref{alg:geoalign} summarizes the full procedure.

% \begin{algorithm*}[t]
% \caption{GeoAlign: Online policy optimization with latent directional consistency}
% \label{alg:geoalign}
% \begin{algorithmic}[1]
% \Require Policy $\pi_\theta$, reward function/model $R$, projector $M_\psi$
% \Require Prompts per batch $N$, rollouts per prompt $K$, projector steps $S$
% \Require Thresholds $(\tau_\alpha, k_{\max})$, $\epsilon$
% \For{$t=1,2,\dots$}
%     \State Sample prompts $\{x_i\}_{i=1}^N\sim\mathcal{D}$
%     \For{$i=1$ to $N$}
%         \State Sample $\{y_{i,k}\}_{k=1}^K\sim\pi_\theta(\cdot\mid x_i)$
%         \For{$k=1$ to $K$}
%             \State $r_{i,k}\gets R(x_i,y_{i,k})$
%             \State $h_{i,k}\gets \textsc{PoolHidden}(\pi_\theta,x_i,y_{i,k})$
%         \EndFor
%     \EndFor
%     \State $\mathcal{B}\gets\{(x_i,y_{i,k},r_{i,k},h_{i,k})\}_{i,k}$

%     \State \textbf{Rectify batch:} $\mathcal{B}_{\mathrm{rect}}\gets \textsc{GeoAlign}(\mathcal{B},M_\psi,S,\tau_\alpha,k_{\max})$
%     \State $\theta \gets \textsc{RL\_Update}(\theta,\mathcal{B}_{\mathrm{rect}})$
% \EndFor
% \vspace{0.25em}

% \Function{\textsc{GeoAlign}}{$\mathcal{B},M_\psi,S,\tau_\alpha,k_{\max}$}
%     \State Construct preference set $\mathcal{P}=\bigcup_i\{(i,k,\ell): r_{i,k}>r_{i,\ell}\}$
%     \State Update $(\psi,w)$ for $S$ steps by minimizing $\mathcal{L}_{\mathrm{map}}$ in Eq.~\eqref{eq:projector}
%     \For{each $(i,k,\ell)\in\mathcal{P}$}
%         \State $\delta_{i,k\ell}\gets M_\psi(h_{i,k}-h_{i,\ell})$;\;
%         $\tilde\delta_{i,k\ell}\gets \delta_{i,k\ell}/(\|\delta_{i,k\ell}\|+\epsilon)$
%     \EndFor
%     \State Compute $v_{\mathrm{proto}}$ by Eq.~\eqref{eq:proto}
%     \State Compute pair anomalies $s_{i,k\ell}$ by Eq.~\eqref{eq:pair-anom}
%     \State Compute rollout scores $\alpha_{i,k}$ by Eq.~\eqref{eq:alpha}
%     \State Flag anomalies $\mathcal{Y}_{\mathrm{anom}}$ by Eq.~\eqref{eq:dual-threshold}
%     \For{each $(i,k)\in\mathcal{Y}_{\mathrm{anom}}$}
%         \State $\mathcal{S}_i\gets\{k':(i,k')\notin\mathcal{Y}_{\mathrm{anom}}\}$
%         \State Sample $k^\star\sim \textsc{BestRandom}(\mathcal{S}_i;\{r_{i,k'}\})$ using Eq.~\eqref{eq:br}
%         \State Replace $(y_{i,k},h_{i,k},r_{i,k})\leftarrow (y_{i,k^\star},h_{i,k^\star},r_{i,k^\star})$
%     \EndFor
%     \State \Return $\mathcal{B}_{\mathrm{rect}}$
% \EndFunction
% \end{algorithmic}
% \end{algorithm*}

% \subsection{Complexity Analysis}
% \label{sec:geoalign-complexity}

% Let $P=|\mathcal{P}|$ be the number of preference pairs per batch. In the worst case,
% $P=N\cdot K(K-1)/2$. GeoAlign reuses forward-pass hidden states and incurs no additional policy backpropagation.

% \paragraph{Time.}
% Computing all projected directions costs $O(P\cdot d')$ for a linear projector (or $O(P\cdot \mathrm{cost}(M_\psi))$
% in general). Prototype and cosine anomalies also cost $O(P\cdot d')$.
% Projector training adds $S$ small-step updates over $O(P\cdot d')$ features, which is typically negligible compared to
% a single policy update step (\TODO{report measured overhead in experiments}).

% \paragraph{Memory.}
% Storing pooled representations requires $O(NK d)$. Storing all pairwise directions explicitly requires $O(P d')$,
% but can be streamed to avoid materializing all pairs (\TODO{state whether you stream or materialize}).

% \paragraph{Practical note.}
% When $K$ is large, one may subsample preference pairs (e.g., top-$m$ winners vs. bottom-$m$ losers per prompt)
% to reduce $P$ without changing the module design (\TODO{state if used}).

% \subsection{Discussion and Implementation Details}
% \label{sec:geoalign-discussion}
% We highlight several design choices and their implications.

% \paragraph{Why representation directions (not gradients).}
% GeoAlign estimates directional consistency in latent space using forward-pass representations only, avoiding
% per-sample gradients or second-order influence computations. This makes it suitable for large-scale online RL where
% thousands of rollouts are generated per iteration.

% \paragraph{Prototype stability.}
% Eq.~\eqref{eq:proto} uses a batch mean of unit directions; this is simple and stable in practice.
% (\TODO{Optional improvement: describe EMA/trimmed mean as a robust variant and include ablations.})

% \paragraph{Resampling vs. weighting.}
% We implement experience calibration via prompt-wise resampling to maintain rollout count and avoid discarding data.
% Alternatively, GeoAlign can be implemented as a soft weight $w_{i,k}=f(\alpha_{i,k})$ multiplying the policy loss
% (\TODO{mention if included as ablation}). Resampling is plug-and-play with existing PPO/GRPO pipelines, while weighting
% provides a more ``on-policy''-faithful intervention.

% \paragraph{Pooling and layer choice.}
% \TODO{Specify which layer and pooling; note whether hidden states are detached (stop-gradient) and whether representations
% come from the current policy or a reference model.}

% \paragraph{Hyperparameters.}
% \TODO{Provide default values: $K,N,S,d',\tau_\alpha,k_{\max}$ and sensitivity notes.}

% }

==> ICML/sec/bak/0123_motivation.tex <==
\section{Motivation}
\label{sec:motivation}

\zhenqing{WIP: re-organize and review method}

% 

\subsection{Preliminary}
\label{subsec:preliminary}

GRPO Appendix~\ref{appendix:algorithm_grpo}


\subsection{Observation and Insight: Why Directional Consistency Helps}

GeoAlign is motivated by a simple geometric perspective on on-policy RL fine-tuning.
Consider one RL iteration with a batch of prompts $\{x_i\}_{i=1}^N$, and $K$ rollouts per prompt sampled from the current policy $\pi_\theta$.
Let $h_\theta(x,y)\in\mathbb{R}^d$ denote a pooled hidden representation of the rollout (e.g., last-layer mean pooling), and define a \emph{preference displacement} for a within-prompt preference pair $(y_w,y_l)$ as
$\delta = h_\theta(x,y_w) - h_\theta(x,y_l)$.

\paragraph{Insight 1 (local improvement directions concentrate).}
If the reward model is approximately consistent within the current batch (i.e., it induces a stable notion of ``better'' for most prompts), then improving reward often corresponds to modifying a limited set of high-level attributes (helpfulness, harmlessness, correctness, etc.).
Under mild smoothness of representations, this implies that, within a single iteration, many preference displacements $\{\delta_j\}_{j\in\mathcal{P}}$ tend to share a dominant direction or a low-dimensional subspace, up to task-irrelevant variation.
Empirically, our online projector $\mathcal{M}_\psi$ makes this concentration explicit by suppressing nuisance factors and producing projected directions that exhibit high cosine agreement (Sec.~\ref{exp:ProjectorNecessary}).

% zt：非常不建议涉及梯度和方差的预设，担心审稿人往往会要求严谨的理论证明或特定的梯度分析实验（目前end-to-end的梯度曲线并没有展现相关特性）。这并非本文的核心贡献。
% \paragraph{Insight 2 (directional outliers inflate update variance).}
% Policy gradient methods update parameters using a weighted average of per-sample learning signals.
% When a small fraction of rollouts induces preference displacements that are nearly orthogonal (or adversarial) to the batch-wise dominant direction, their corresponding gradient contributions behave like \emph{high-leverage} points: they can substantially rotate the aggregated update direction and increase update variance, causing oscillatory training dynamics even if their scalar rewards are high.
% Importantly, PPO/GRPO clipping constrains the \emph{magnitude} of each sample's contribution through probability ratios, but does not prevent a small set of samples from rotating the aggregated update direction.

\paragraph{Insight 2 (directional outliers signal spurious improvement).} While scalar rewards indicate \textit{how much} a response is preferred, the latent direction indicates \textit{why}. Samples that achieve high rewards but exhibit improvement directions orthogonal to the consensus manifold are likely exploiting spurious correlations or specific quirks of the reward proxy (i.e., reward hacking), rather than learning the intended task. Relying on these idiosyncratic trajectories risks overfitting to the proxy, whereas the consensus direction represents the robust, generalizable path of policy improvement.

\paragraph{Insight 3 (GeoAlign as robust estimation).}
Viewed abstractly, one iteration of policy optimization can be seen as estimating a latent ``consensus improvement'' direction from noisy directional observations.
GeoAlign computes a consensus prototype $v_{\mathrm{proto}}$ and suppresses rollouts with large angular deviation from it, analogous to robust $M$-estimation where outliers receive bounded influence.
This perspective explains why GeoAlign improves stability under reward corruption: directionally inconsistent samples are treated as outliers in the space of improvement directions, rather than being trusted solely based on scalar reward values.

\subsection{Challenge and Target}



